Multiplicity dependence of light-flavor hadron production in pp collisions at $\sqrt{s}$ = 7 TeV

Comprehensive results on the production of unidentified charged particles, $\pi^{\pm}$, $\rm{K}^{\pm}$, $\rm{K}^{0}_{S}$, $\rm{K}$*(892)$^{0}$, $\rm{p}$, $\overline{\rm{p}}$, $\phi$(1020), $\Lambda$, $\overline{\Lambda}$, $\Xi^{-}$, $\overline{\Xi}^{+}$, $\Omega^{-}$ and $\overline{\Omega}^{+}$ hadrons in proton-proton (pp) collisions at $\sqrt{s}$ = 7 TeV at midrapidity ($|y| < 0.5$) as a function of charged-particle multiplicity density are presented. In order to avoid auto-correlation biases, the actual transverse momentum ($p_{\rm{T}}$) spectra of the particles under study and the event activity are measured in different rapidity windows. In the highest multiplicity class, the charged-particle density reaches about 3.5 times the value measured in inelastic collisions. While the yield of protons normalized to pions remains approximately constant as a function of multiplicity, the corresponding ratios of strange hadrons to pions show a significant enhancement that increases with increasing strangeness content. Furthermore, all identified particle to pion ratios are shown to depend solely on charged-particle multiplicity density, regardless of system type and collision energy. The evolution of the spectral shapes with multiplicity and hadron mass shows patterns that are similar to those observed in p-Pb and Pb-Pb collisions at LHC energies. The obtained $p_{\rm{T}}$ distributions and yields are compared to expectations from QCD-based pp event generators as well as to predictions from thermal and hydrodynamic models. These comparisons indicate that traces of a collective, equilibrated system are already present in high-multiplicity pp collisions.

==> tables/yieldmean_tables.tex <==

 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $\pi^{+} + \pi^{-}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanPionSum_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$\pi^{+} + \pi^{-}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--100\% & $(5952.5\pm0.5\pm299.4)\times10^{-3}$ & $(4602.8\pm0.5\pm124.7)\times10^{-4}$ \\ 
0--1\% & $(200.7\pm0.1\pm10.3(3.9))\times10^{-1}$ & $(535.7\pm0.3\pm14.4(3.2))\times10^{-3}$ \\ 
1--5\% & $(1575.5\pm0.4\pm75.6(24.2))\times10^{-2}$ & $(515.6\pm0.1\pm13.6(2.2))\times10^{-3}$ \\ 
5--10\% & $(1291.7\pm0.3\pm61.3(20.4))\times10^{-2}$ & $(500.6\pm0.1\pm13.2(2.2))\times10^{-3}$ \\ 
10--15\% & $(1110.7\pm0.2\pm52.6(17.8))\times10^{-2}$ & $(489.6\pm0.1\pm13.0(2.2))\times10^{-3}$ \\ 
15--20\% & $(978.4\pm0.2\pm46.3(16.1))\times10^{-2}$ & $(480.4\pm0.1\pm12.7(2.3))\times10^{-3}$ \\ 
20--30\% & $(827.5\pm0.1\pm39.2(13.5))\times10^{-2}$ & $(4691.7\pm0.9\pm124.8(21.9))\times10^{-4}$ \\ 
30--40\% & $(665.0\pm0.1\pm31.3(11.1))\times10^{-2}$ & $(4556.0\pm0.9\pm120.3(21.5))\times10^{-4}$ \\ 
40--50\% & $(539.5\pm0.1\pm25.6(8.9))\times10^{-2}$ & $(4425.6\pm1.0\pm116.7(20.5))\times10^{-4}$ \\ 
50--70\% & $(3974.6\pm0.6\pm212.6(64.6))\times10^{-3}$ & $(4236.9\pm0.8\pm115.4(18.7))\times10^{-4}$ \\ 
70--100\% & $(2418.0\pm0.4\pm174.1(39.4))\times10^{-3}$ & $(3904.1\pm0.7\pm116.6(16.6))\times10^{-4}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $K^{+} + K^{-}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanKaonSum_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$K^{+} + K^{-}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--100\% & $(758.1\pm0.2\pm49.1)\times10^{-3}$ & $(768.9\pm0.1\pm19.9)\times10^{-3}$ \\ 
0--1\% & $(274.7\pm0.6\pm18.7(7.4))\times10^{-2}$ & $(933.3\pm0.9\pm19.2(7.1))\times10^{-3}$ \\ 
1--5\% & $(212.3\pm0.2\pm13.6(5.1))\times10^{-2}$ & $(889.3\pm0.4\pm18.6(6.1))\times10^{-3}$ \\ 
5--10\% & $(171.8\pm0.2\pm10.9(4.3))\times10^{-2}$ & $(855.9\pm0.4\pm18.8(6.5))\times10^{-3}$ \\ 
10--15\% & $(146.1\pm0.1\pm9.2(3.6))\times10^{-2}$ & $(831.8\pm0.4\pm18.9(6.5))\times10^{-3}$ \\ 
15--20\% & $(127.7\pm0.1\pm8.0(3.2))\times10^{-2}$ & $(811.4\pm0.4\pm19.0(6.8))\times10^{-3}$ \\ 
20--30\% & $(1067.1\pm0.7\pm67.0(27.2))\times10^{-3}$ & $(786.8\pm0.3\pm19.1(7.1))\times10^{-3}$ \\ 
30--40\% & $(845.9\pm0.6\pm53.0(22.2))\times10^{-3}$ & $(754.0\pm0.3\pm19.2(7.5))\times10^{-3}$ \\ 
40--50\% & $(676.3\pm0.5\pm42.7(18.1))\times10^{-3}$ & $(723.3\pm0.4\pm19.3(7.9))\times10^{-3}$ \\ 
50--70\% & $(485.6\pm0.3\pm33.2(13.5))\times10^{-3}$ & $(675.7\pm0.3\pm20.1(8.7))\times10^{-3}$ \\ 
70--100\% & $(280.3\pm0.2\pm23.7(8.4))\times10^{-3}$ & $(588.7\pm0.3\pm21.5(9.9))\times10^{-3}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $p + \bar{p}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanProtonSum_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$p + \bar{p}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--100\% & $(324.4\pm0.2\pm23.9)\times10^{-3}$ & $(896.2\pm0.3\pm30.4)\times10^{-3}$ \\ 
0--1\% & $(109.8\pm0.2\pm8.1(3.3))\times10^{-2}$ & $(113.5\pm0.1\pm2.9(1.1))\times10^{-2}$ \\ 
1--5\% & $(87.4\pm0.1\pm6.2(2.5))\times10^{-2}$ & $(1070.7\pm0.7\pm28.3(10.8))\times10^{-3}$ \\ 
5--10\% & $(719.8\pm0.8\pm50.9(21.2))\times10^{-3}$ & $(1020.5\pm0.7\pm28.3(10.8))\times10^{-3}$ \\ 
10--15\% & $(621.1\pm0.7\pm44.0(18.8))\times10^{-3}$ & $(981.6\pm0.7\pm28.4(11.1))\times10^{-3}$ \\ 
15--20\% & $(548.2\pm0.6\pm38.9(17.0))\times10^{-3}$ & $(953.9\pm0.7\pm28.5(11.5))\times10^{-3}$ \\ 
20--30\% & $(463.2\pm0.4\pm33.0(14.7))\times10^{-3}$ & $(917.1\pm0.6\pm28.6(11.9))\times10^{-3}$ \\ 
30--40\% & $(371.9\pm0.3\pm26.7(12.3))\times10^{-3}$ & $(872.6\pm0.6\pm28.9(12.7))\times10^{-3}$ \\ 
40--50\% & $(298.1\pm0.3\pm21.7(10.3))\times10^{-3}$ & $(828.6\pm0.6\pm29.2(13.6))\times10^{-3}$ \\ 
50--70\% & $(213.9\pm0.2\pm16.9(7.9))\times10^{-3}$ & $(771.8\pm0.5\pm30.2(15.0))\times10^{-3}$ \\ 
70--100\% & $(117.0\pm0.1\pm11.5(5.2))\times10^{-3}$ & $(664.9\pm0.4\pm32.4(18.0))\times10^{-3}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $K^{0}_{S}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanK0Short_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$K^{0}_{S}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--100\% & $(374.0\pm0.4\pm20.5)\times10^{-3}$ & $(774.0\pm0.6\pm10.8)\times10^{-3}$ \\ 
0--1\% & $(133.7\pm0.4\pm7.0(3.2))\times10^{-2}$ & $(93.7\pm0.2\pm1.2(0.6))\times10^{-2}$ \\ 
1--5\% & $(104.0\pm0.2\pm5.4(2.5))\times10^{-2}$ & $(89.1\pm0.1\pm1.2(0.5))\times10^{-2}$ \\ 
5--10\% & $(84.1\pm0.2\pm4.4(2.0))\times10^{-2}$ & $(86.1\pm0.1\pm1.1(0.5))\times10^{-2}$ \\ 
10--15\% & $(71.9\pm0.2\pm3.7(1.7))\times10^{-2}$ & $(83.5\pm0.1\pm1.1(0.5))\times10^{-2}$ \\ 
15--20\% & $(62.9\pm0.1\pm3.3(1.5))\times10^{-2}$ & $(81.5\pm0.2\pm1.0(0.5))\times10^{-2}$ \\ 
20--30\% & $(527.8\pm1.0\pm27.5(12.9))\times10^{-3}$ & $(78.9\pm0.1\pm1.0(0.5))\times10^{-2}$ \\ 
30--40\% & $(419.6\pm0.9\pm21.9(10.5))\times10^{-3}$ & $(75.5\pm0.1\pm1.0(0.5))\times10^{-2}$ \\ 
40--50\% & $(334.3\pm0.8\pm17.8(9.1))\times10^{-3}$ & $(72.8\pm0.1\pm0.9(0.5))\times10^{-2}$ \\ 
50--70\% & $(239.2\pm0.5\pm14.6(9.7))\times10^{-3}$ & $(68.3\pm0.1\pm1.0(0.7))\times10^{-2}$ \\ 
70--100\% & $(130.7\pm0.3\pm11.1(9.3))\times10^{-3}$ & $(60.4\pm0.1\pm1.2(1.0))\times10^{-2}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $\Lambda + \bar{\Lambda}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanLambdaSum_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$\Lambda + \bar{\Lambda}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--100\% & $(205.0\pm0.3\pm15.5)\times10^{-3}$ & $(1024.2\pm1.0\pm37.0)\times10^{-3}$ \\ 
0--1\% & $(77.5\pm0.3\pm5.4(2.8))\times10^{-2}$ & $(127.7\pm0.3\pm3.9(3.0))\times10^{-2}$ \\ 
1--5\% & $(60.5\pm0.1\pm4.2(2.2))\times10^{-2}$ & $(120.1\pm0.2\pm3.8(2.9))\times10^{-2}$ \\ 
5--10\% & $(48.9\pm0.1\pm3.5(2.0))\times10^{-2}$ & $(114.4\pm0.2\pm3.8(3.1))\times10^{-2}$ \\ 
10--15\% & $(41.5\pm0.1\pm3.0(1.9))\times10^{-2}$ & $(110.2\pm0.2\pm3.8(3.3))\times10^{-2}$ \\ 
15--20\% & $(361.8\pm0.9\pm26.5(16.4))\times10^{-3}$ & $(106.8\pm0.2\pm3.7(3.1))\times10^{-2}$ \\ 
20--30\% & $(300.1\pm0.7\pm22.2(14.8))\times10^{-3}$ & $(102.6\pm0.1\pm3.7(3.3))\times10^{-2}$ \\ 
30--40\% & $(236.4\pm0.6\pm18.1(12.8))\times10^{-3}$ & $(97.5\pm0.1\pm3.7(3.3))\times10^{-2}$ \\ 
40--50\% & $(184.7\pm0.6\pm14.4(9.3))\times10^{-3}$ & $(92.8\pm0.2\pm3.6(3.1))\times10^{-2}$ \\ 
50--70\% & $(125.6\pm0.3\pm11.0(8.4))\times10^{-3}$ & $(86.6\pm0.1\pm3.6(3.2))\times10^{-2}$ \\ 
70--100\% & $(58.3\pm0.2\pm7.1(6.3))\times10^{-3}$ & $(75.6\pm0.1\pm3.8(3.6))\times10^{-2}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $\Xi^{-} + \bar{\Xi}^{+}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanXiSum_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$\Xi^{-} + \bar{\Xi}^{+}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--1\% & $(9.7\pm0.2\pm0.7(0.4))\times10^{-2}$ & $(14.6\pm0.1\pm0.2(0.1))\times10^{-1}$ \\ 
1--5\% & $(72.4\pm0.8\pm5.5(3.6))\times10^{-3}$ & $(137.6\pm0.7\pm2.0(1.0))\times10^{-2}$ \\ 
5--10\% & $(59.9\pm0.6\pm4.8(3.4))\times10^{-3}$ & $(128.8\pm0.7\pm1.9(0.9))\times10^{-2}$ \\ 
10--15\% & $(48.8\pm0.6\pm4.0(2.9))\times10^{-3}$ & $(126.3\pm0.7\pm1.8(1.1))\times10^{-2}$ \\ 
15--20\% & $(41.0\pm0.5\pm3.5(2.6))\times10^{-3}$ & $(122.7\pm0.8\pm1.8(1.1))\times10^{-2}$ \\ 
20--30\% & $(33.5\pm0.4\pm3.0(2.2))\times10^{-3}$ & $(118.5\pm0.6\pm1.7(0.8))\times10^{-2}$ \\ 
30--40\% & $(25.0\pm0.3\pm2.3(1.8))\times10^{-3}$ & $(113.8\pm0.7\pm1.6(0.8))\times10^{-2}$ \\ 
40--50\% & $(18.9\pm0.3\pm1.9(1.6))\times10^{-3}$ & $(109.1\pm0.8\pm1.9(1.7))\times10^{-2}$ \\ 
50--70\% & $(12.0\pm0.2\pm1.4(1.2))\times10^{-3}$ & $(101.3\pm0.7\pm1.9(1.9))\times10^{-2}$ \\ 
70--100\% & $(51.4\pm1.0\pm7.4(6.7))\times10^{-4}$ & $(90.0\pm1.0\pm2.2(1.9))\times10^{-2}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
 
\begin{table}
\caption{Integrated yields ($dN/dy$) and average transverse momentum ($\langle p_{\mathrm{T}} \rangle$) for $\Omega^{-} + \bar{\Omega}^{+}$ at midrapidity ($|y|<1.0$) in pp collisions at 7 TeV. Uncertainties are statistical and total($N_{ch}$-dependent) systematics, respectively.}
\label{tab:YieldMeanOmegaSum_}
\begin{center}
\begin{tabular}{ c | c c }
\hline
\multirow{2}{*}{V0M Multiplicity Class} & \multicolumn{2}{c}{$\Omega^{-} + \bar{\Omega}^{+}$} \\ 
& $dN/dy$ & $\langle p_{\mathrm{T}} \rangle$ (GeV/\textit{c})\\ 
\hline
0--5\% & $(8.6\pm0.3\pm0.7(0.5))\times10^{-3}$ & $(16.2\pm0.2\pm0.3(0.2))\times10^{-1}$ \\ 
5--15\% & $(5.3\pm0.2\pm0.5(0.3))\times10^{-3}$ & $(15.4\pm0.3\pm0.3(0.2))\times10^{-1}$ \\ 
15--30\% & $(3.1\pm0.1\pm0.3(0.2))\times10^{-3}$ & $(14.5\pm0.3\pm0.2(0.2))\times10^{-1}$ \\ 
30--50\% & $(1.9\pm0.1\pm0.2(0.2))\times10^{-3}$ & $(12.8\pm0.4\pm0.3(0.2))\times10^{-1}$ \\ 
50--100\% & $(5.5\pm0.5\pm0.8(0.7))\times10^{-4}$ & $(11.4\pm0.6\pm0.3(0.3))\times10^{-1}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}
